Audio-to-Score Alignment Using Deep Automatic Music Transcription

Audio-to-score alignment (A2SA) is a multimodal task consisting in the alignment of audio signals to music scores. Recent literature confirms the benefits of Automatic Music Transcription (AMT) for A2SA at the frame-level. In this work, we aim to elaborate on the exploitation of AMT Deep Learning (DL) models for achieving alignment at the note-level. We propose a method which benefits from HMM-based score-to-score alignment and AMT, showing a remarkable advancement beyond the state-of-the-art. We design a systematic procedure to take advantage of large datasets which do not offer an aligned score. Finally, we perform a thorough comparison and extensive tests on multiple datasets.

==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_OUTPUT_EXCMD	mixed	/number, pattern, mixed, or combineV2/
!_TAG_OUTPUT_FILESEP	slash	/slash or backslash/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PATTERN_LENGTH_LIMIT	96	/0 for no limit/
!_TAG_PROC_CWD	/home/sapo/Develop/phd/alignment/mmsp2021/	//
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	5.9.0	/p5.9.20210110.0/
IEEE_J_AC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_AC         = "{IEEE} Trans. Autom. Control"}$/;"	s
IEEE_J_AC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_AC         = "{IEEE} Transactions on Automatic Control"}$/;"	s
IEEE_J_ADVP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_ADVP       = "{IEEE} Trans. Adv. Packag."}$/;"	s
IEEE_J_ADVP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_ADVP       = "{IEEE} Transactions on Advanced Packaging"}$/;"	s
IEEE_J_AES	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_AES        = "{IEEE} Trans. Aerosp. Electron. Syst."}$/;"	s
IEEE_J_AES	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_AES        = "{IEEE} Transactions on Aerospace and Electronic Systems"}$/;"	s
IEEE_J_AIRE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_AIRE       = "{IEEE} Trans. Airborne Electron."}$/;"	s
IEEE_J_AIRE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_AIRE       = "{IEEE} Transactions on Airborne Electronics"}$/;"	s
IEEE_J_ANE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_ANE        = "{IEEE} Trans. Aerosp. Navig. Electron."}$/;"	s
IEEE_J_ANE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_ANE        = "{IEEE} Transactions on Aerospace and Navigational Electronics"}$/;"	s
IEEE_J_ANNE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_ANNE       = "{IEEE} Trans. Aeronaut. Navig. Electron."}$/;"	s
IEEE_J_ANNE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_ANNE       = "{IEEE} Transactions on Aeronautical and Navigational Electronics"}$/;"	s
IEEE_J_AP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_AP         = "{IEEE} Trans. Antennas Propag."}$/;"	s
IEEE_J_AP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_AP         = "{IEEE} Transactions on Antennas and Propagation"}$/;"	s
IEEE_J_APPIND	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_APPIND     = "{IEEE} Trans. Appl. Ind."}$/;"	s
IEEE_J_APPIND	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_APPIND     = "{IEEE} Transactions on Applications and Industry"}$/;"	s
IEEE_J_AS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_AS         = "{IEEE} Trans. Aerosp."}$/;"	s
IEEE_J_AS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_AS         = "{IEEE} Transactions on Aerospace"}$/;"	s
IEEE_J_ASC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_ASC        = "{IEEE} Trans. Appl. Supercond."}$/;"	s
IEEE_J_ASC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_ASC        = "{IEEE} Transactions on Applied Superconductivity"}$/;"	s
IEEE_J_ASE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_ASE        = "{IEEE} Trans. Autom. Sci. Eng."}$/;"	s
IEEE_J_ASE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_ASE        = "{IEEE} Transactions on Automation Science and Engineering"}$/;"	s
IEEE_J_ASSP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_ASSP       = "{IEEE} Trans. Acoust., Speech, Signal Process."}$/;"	s
IEEE_J_ASSP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_ASSP       = "{IEEE} Transactions on Acoustics, Speech, and Signal Processing"}$/;"	s
IEEE_J_AU	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_AU         = "{IEEE} Trans. Audio"}$/;"	s
IEEE_J_AU	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_AU         = "{IEEE} Transactions on Audio"}$/;"	s
IEEE_J_AUEA	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_AUEA       = "{IEEE} Trans. Audio Electroacoust."}$/;"	s
IEEE_J_AUEA	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_AUEA       = "{IEEE} Transactions on Audio and Electroacoustics"}$/;"	s
IEEE_J_AWPL	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_AWPL       = "{IEEE} Antennas Wireless Propag. Lett."}$/;"	s
IEEE_J_AWPL	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_AWPL       = "{IEEE} Antennas and Wireless Propagation Letters"}$/;"	s
IEEE_J_B-ME	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_B-ME       = "{IEEE} Trans. Bio-Med. Eng."}$/;"	s
IEEE_J_B-ME	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_B-ME       = "{IEEE} Transactions on Bio-Medical Engineering"}$/;"	s
IEEE_J_BC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_BC         = "{IEEE} Trans. Broadcast."}$/;"	s
IEEE_J_BC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_BC         = "{IEEE} Transactions on Broadcasting"}$/;"	s
IEEE_J_BCTV	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_BCTV       = "{IEEE} Transactions on Broadcast and Television Receivers"}$/;"	s
IEEE_J_BME	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_BME        = "{IEEE} Trans. Biomed. Eng."}$/;"	s
IEEE_J_BME	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_BME        = "{IEEE} Transactions on Biomedical Engineering"}$/;"	s
IEEE_J_BMELC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_BMELC      = "{IEEE} Trans. Bio-Med. Electron."}$/;"	s
IEEE_J_BMELC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_BMELC      = "{IEEE} Transactions on Bio-Medical Electronics"}$/;"	s
IEEE_J_C	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_C          = "{IEEE} Trans. Comput."}$/;"	s
IEEE_J_C	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_C          = "{IEEE} Transactions on Computers"}$/;"	s
IEEE_J_CAD	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CAD        = "{IEEE} Trans. Comput.-Aided Design Integr. Circuits Syst."}$/;"	s
IEEE_J_CAD	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CAD        = "{IEEE} Transactions on Computer-Aided Design of Integrated Circuits/;"	s
IEEE_J_CAL	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CAL        = "{IEEE} Comput. Archit. Lett."}$/;"	s
IEEE_J_CAL	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CAL        = "{IEEE} Computer Architecture Letters"}$/;"	s
IEEE_J_CAPT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CAPT       = "{IEEE} Trans. Compon. Packag. Technol."}$/;"	s
IEEE_J_CAPT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CAPT       = "{IEEE} Transactions on Components and Packaging Technology"}$/;"	s
IEEE_J_CAPTS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CAPTS      = "{IEEE} Trans. Compon. Packag. Technol."}$/;"	s
IEEE_J_CAPTS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CAPTS      = "{IEEE} Transactions on Components and Packaging Technologies"}$/;"	s
IEEE_J_CAS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CAS        = "{IEEE} Trans. Circuits Syst."}$/;"	s
IEEE_J_CAS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CAS        = "{IEEE} Transactions on Circuits and Systems"}$/;"	s
IEEE_J_CASI	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CASI       = "{IEEE} Trans. Circuits Syst. {I}"}$/;"	s
IEEE_J_CASI	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CASI       = "{IEEE} Transactions on Circuits and Systems---Part {I}: Fundamental/;"	s
IEEE_J_CASII	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CASII      = "{IEEE} Trans. Circuits Syst. {II}"}$/;"	s
IEEE_J_CASII	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CASII      = "{IEEE} Transactions on Circuits and Systems---Part {II}: Analog and/;"	s
IEEE_J_CASII_EB	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CASII_EB   = "{IEEE} Trans. Circuits Syst. {II}"}$/;"	s
IEEE_J_CASII_EB	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CASII_EB   = "{IEEE} Transactions on Circuits and Systems---Part {II}: Express Br/;"	s
IEEE_J_CASI_RP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CASI_RP    = "{IEEE} Trans. Circuits Syst. {I}"}$/;"	s
IEEE_J_CASI_RP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CASI_RP    = "{IEEE} Transactions on Circuits and Systems---Part {I}: Regular Pap/;"	s
IEEE_J_CASVT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CASVT      = "{IEEE} Trans. Circuits Syst. Video Technol."}$/;"	s
IEEE_J_CASVT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CASVT      = "{IEEE} Transactions on Circuits and Systems for Video Technology"}$/;"	s
IEEE_J_CBB	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CBB        = "{IEEE\/ACM} Transactions on Computational Biology and Bioinformatic/;"	s
IEEE_J_CE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CE         = "{IEEE} Trans. Consum. Electron."}$/;"	s
IEEE_J_CE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CE         = "{IEEE} Transactions on Consumer Electronics"}$/;"	s
IEEE_J_CHMT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CHMT       = "{IEEE} Trans. Compon., Hybrids, Manuf. Technol."}$/;"	s
IEEE_J_CHMT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CHMT       = "{IEEE} Transactions on Components, Hybrids and Manufacturing Techno/;"	s
IEEE_J_CJECE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CJECE      = "Canadian Journal of Electrical and Computer Engineering"}$/;"	s
IEEE_J_COM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_COM        = "{IEEE} Trans. Commun."}$/;"	s
IEEE_J_COM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_COM        = "{IEEE} Transactions on Communications"}$/;"	s
IEEE_J_COML	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_COML       = "{IEEE} Commun. Lett."}$/;"	s
IEEE_J_COML	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_COML       = "{IEEE} Communications Letters"}$/;"	s
IEEE_J_COMT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_COMT       = "{IEEE} Trans. Commun. Technol."}$/;"	s
IEEE_J_COMT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_COMT       = "{IEEE} Transactions on Communication Technology"}$/;"	s
IEEE_J_CPART	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CPART      = "{IEEE} Trans. Compon. Parts"}$/;"	s
IEEE_J_CPART	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CPART      = "{IEEE} Transactions on Component Parts"}$/;"	s
IEEE_J_CPMTA	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CPMTA      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {A}"}$/;"	s
IEEE_J_CPMTA	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CPMTA      = "{IEEE} Transactions on Components, Packaging and Manufacturing Tech/;"	s
IEEE_J_CPMTB	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CPMTB      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {B}"}$/;"	s
IEEE_J_CPMTB	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CPMTB      = "{IEEE} Transactions on Components, Packaging and Manufacturing Tech/;"	s
IEEE_J_CPMTC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CPMTC      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {C}"}$/;"	s
IEEE_J_CPMTC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CPMTC      = "{IEEE} Transactions on Components, Packaging and Manufacturing Tech/;"	s
IEEE_J_CST	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CST        = "{IEEE} Trans. Control Syst. Technol."}$/;"	s
IEEE_J_CST	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CST        = "{IEEE} Transactions on Control Systems Technology"}$/;"	s
IEEE_J_CT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_CT         = "{IEEE} Trans. Circuit Theory"}$/;"	s
IEEE_J_CT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_CT         = "{IEEE} Transactions on Circuit Theory"}$/;"	s
IEEE_J_DEI	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_DEI        = "{IEEE} Trans. Dielectr. Electr. Insul."}$/;"	s
IEEE_J_DEI	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_DEI        = "{IEEE} Transactions on Dielectrics and Electrical Insulation"}$/;"	s
IEEE_J_DMR	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_DMR        = "{IEEE} Trans. Device Mater. Rel."}$/;"	s
IEEE_J_DMR	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_DMR        = "{IEEE} Transactions on Device and Materials Reliability"}$/;"	s
IEEE_J_DSC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_DSC        = "{IEEE} Transactions on Dependable and Secure Computing"}$/;"	s
IEEE_J_EC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_EC         = "{IEEE} Trans. Energy Convers."}$/;"	s
IEEE_J_EC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_EC         = "{IEEE} Transactions on Energy Conversion"}$/;"	s
IEEE_J_ECOMP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_ECOMP      = "{IEEE} Trans. Electron. Comput."}$/;"	s
IEEE_J_ECOMP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_ECOMP      = "{IEEE} Transactions on Electronic Computers"}$/;"	s
IEEE_J_ED	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_ED         = "{IEEE} Trans. Electron Devices"}$/;"	s
IEEE_J_ED	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_ED         = "{IEEE} Transactions on Electron Devices"}$/;"	s
IEEE_J_EDL	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_EDL        = "{IEEE} Electron Device Lett."}$/;"	s
IEEE_J_EDL	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_EDL        = "{IEEE} Electron Device Letters"}$/;"	s
IEEE_J_EDU	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_EDU        = "{IEEE} Trans. Educ."}$/;"	s
IEEE_J_EDU	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_EDU        = "{IEEE} Transactions on Education"}$/;"	s
IEEE_J_EI	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_EI         = "{IEEE} Trans. Electr. Insul."}$/;"	s
IEEE_J_EI	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_EI         = "{IEEE} Transactions on Electrical Insulation"}$/;"	s
IEEE_J_EM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_EM         = "{IEEE} Trans. Eng. Manag."}$/;"	s
IEEE_J_EM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_EM         = "{IEEE} Transactions on Engineering Management"}$/;"	s
IEEE_J_EMC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_EMC        = "{IEEE} Trans. Electromagn. Compat."}$/;"	s
IEEE_J_EMC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_EMC        = "{IEEE} Transactions on Electromagnetic Compatibility"}$/;"	s
IEEE_J_EPM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_EPM        = "{IEEE} Trans. Electron. Packag. Manuf."}$/;"	s
IEEE_J_EPM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_EPM        = "{IEEE} Transactions on Electronics Packaging Manufacturing"}$/;"	s
IEEE_J_ESSL	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_ESSL       = "{IEEE\/ECS} Electrochem. Solid-State Lett."}$/;"	s
IEEE_J_ESSL	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_ESSL       = "{IEEE\/ECS} Electrochemical and Solid-State Letters"}$/;"	s
IEEE_J_EVC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_EVC        = "{IEEE} Trans. Evol. Comput."}$/;"	s
IEEE_J_EVC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_EVC        = "{IEEE} Transactions on Evolutionary Computation"}$/;"	s
IEEE_J_EWS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_EWS        = "{IEEE} Transactions on Engineering Writing and Speech"}$/;"	s
IEEE_J_FUZZ	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_FUZZ       = "{IEEE} Trans. Fuzzy Syst."}$/;"	s
IEEE_J_FUZZ	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_FUZZ       = "{IEEE} Transactions on Fuzzy Systems"}$/;"	s
IEEE_J_GE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_GE         = "{IEEE} Trans. Geosci. Electron."}$/;"	s
IEEE_J_GE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_GE         = "{IEEE} Transactions on Geoscience Electronics"}$/;"	s
IEEE_J_GRS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_GRS        = "{IEEE} Trans. Geosci. Remote Sens."}$/;"	s
IEEE_J_GRS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_GRS        = "{IEEE} Transactions on Geoscience and Remote Sensing"}$/;"	s
IEEE_J_GRSL	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_GRSL       = "{IEEE} Geosci. Remote Sens. Lett."}$/;"	s
IEEE_J_GRSL	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_GRSL       = "{IEEE} Geoscience and Remote Sensing Letters"}$/;"	s
IEEE_J_HFE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_HFE        = "{IEEE} Trans. Hum. Factors Electron."}$/;"	s
IEEE_J_HFE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_HFE        = "{IEEE} Transactions on Human Factors in Electronics"}$/;"	s
IEEE_J_IA	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_IA         = "{IEEE} Trans. Ind. Appl."}$/;"	s
IEEE_J_IA	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_IA         = "{IEEE} Transactions on Industry Applications"}$/;"	s
IEEE_J_IE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_IE         = "{IEEE} Trans. Ind. Electron."}$/;"	s
IEEE_J_IE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_IE         = "{IEEE} Transactions on Industrial Electronics"}$/;"	s
IEEE_J_IECI	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_IECI       = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}$/;"	s
IEEE_J_IECI	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_IECI       = "{IEEE} Transactions on Industrial Electronics and Control Instrumen/;"	s
IEEE_J_IFS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_IFS        = "{IEEE} Trans. Inf. Forensics Security"}$/;"	s
IEEE_J_IFS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_IFS        = "{IEEE} Transactions on Information Forensics and Security"}$/;"	s
IEEE_J_IGA	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_IGA        = "{IEEE} Trans. Ind. Gen. Appl."}$/;"	s
IEEE_J_IGA	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_IGA        = "{IEEE} Transactions on Industry and General Applications"}$/;"	s
IEEE_J_IINF	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_IINF       = "{IEEE} Trans. Ind. Informat."}$/;"	s
IEEE_J_IINF	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_IINF       = "{IEEE} Transactions on Industrial Informatics"}$/;"	s
IEEE_J_IM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_IM         = "{IEEE} Trans. Instrum. Meas."}$/;"	s
IEEE_J_IM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_IM         = "{IEEE} Transactions on Instrumentation and Measurement"}$/;"	s
IEEE_J_IP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_IP         = "{IEEE} Trans. Image Process."}$/;"	s
IEEE_J_IP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_IP         = "{IEEE} Transactions on Image Processing"}$/;"	s
IEEE_J_IT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_IT         = "{IEEE} Trans. Inf. Theory"}$/;"	s
IEEE_J_IT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_IT         = "{IEEE} Transactions on Information Theory"}$/;"	s
IEEE_J_ITBM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_ITBM       = "{IEEE} Trans. Inf. Technol. Biomed."}$/;"	s
IEEE_J_ITBM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_ITBM       = "{IEEE} Transactions on Information Technology in Biomedicine"}$/;"	s
IEEE_J_ITS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_ITS        = "{IEEE} Trans. Intell. Transp. Syst."}$/;"	s
IEEE_J_ITS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_ITS        = "{IEEE} Transactions on Intelligent Transportation Systems"}$/;"	s
IEEE_J_JDT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_JDT        = "{IEEE\/OSA} J. Display Technol."}$/;"	s
IEEE_J_JDT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_JDT        = "{IEEE\/OSA} Journal of Display Technology"}$/;"	s
IEEE_J_JEM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_JEM        = "{IEEE\/TMS} J. Electron. Mater."}$/;"	s
IEEE_J_JEM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_JEM        = "{IEEE\/TMS} Journal of Electronic Materials"}$/;"	s
IEEE_J_JLT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_JLT        = "J. Lightw. Technol."}$/;"	s
IEEE_J_JLT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_JLT        = "{IEEE\/OSA} Journal of Lightwave Technology"}$/;"	s
IEEE_J_JQE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_JQE        = "{IEEE} J. Quantum Electron."}$/;"	s
IEEE_J_JQE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_JQE        = "{IEEE} Journal of Quantum Electronics"}$/;"	s
IEEE_J_JRA	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_JRA        = "{IEEE} J. Robot. Autom."}$/;"	s
IEEE_J_JRA	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_JRA        = "{IEEE} Journal of Robotics and Automation"}$/;"	s
IEEE_J_JSAC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_JSAC       = "{IEEE} J. Sel. Areas Commun."}$/;"	s
IEEE_J_JSAC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_JSAC       = "{IEEE} Journal on Selected Areas in Communications"}$/;"	s
IEEE_J_JSSC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_JSSC       = "{IEEE} J. Solid-State Circuits"}$/;"	s
IEEE_J_JSSC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_JSSC       = "{IEEE} Journal of Solid-State Circuits"}$/;"	s
IEEE_J_JSTQE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_JSTQE      = "{IEEE} J. Sel. Topics Quantum Electron."}$/;"	s
IEEE_J_JSTQE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_JSTQE      = "{IEEE} Journal of Selected Topics in Quantum Electronics"}$/;"	s
IEEE_J_KDE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_KDE        = "{IEEE} Trans. Knowl. Data Eng."}$/;"	s
IEEE_J_KDE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_KDE        = "{IEEE} Transactions on Knowledge and Data Engineering"}$/;"	s
IEEE_J_MAG	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}$/;"	s
IEEE_J_MAG	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_MAG        = "{IEEE} Transactions on Magnetics"}$/;"	s
IEEE_J_MC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_MC         = "{IEEE} Trans. Mobile Comput."}$/;"	s
IEEE_J_MC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_MC         = "{IEEE} Transactions on Mobile Computing"}$/;"	s
IEEE_J_ME	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_ME         = "{IEEE} Trans. Med. Electron."}$/;"	s
IEEE_J_ME	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_ME         = "{IEEE} Transactions on Medical Electronics"}$/;"	s
IEEE_J_MECH	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_MECH       = "{IEEE\/ASME} Trans. Mechatronics"}$/;"	s
IEEE_J_MECH	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_MECH       = "{IEEE\/ASME} Transactions on Mechatronics"}$/;"	s
IEEE_J_MEMS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_MEMS       = "J. Microelectromech. Syst."}$/;"	s
IEEE_J_MEMS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_MEMS       = "{IEEE\/ASME} Journal of Microelectromechanical Systems"}$/;"	s
IEEE_J_MFT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_MFT        = "{IEEE} Trans. Manuf. Technol."}$/;"	s
IEEE_J_MFT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_MFT        = "{IEEE} Transactions on Manufacturing Technology"}$/;"	s
IEEE_J_MGWL	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_MGWL       = "{IEEE} Microw. Guided Wave Lett."}$/;"	s
IEEE_J_MGWL	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_MGWL       = "{IEEE} Microwave and Guided Wave Letters"}$/;"	s
IEEE_J_MI	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_MI         = "{IEEE} Trans. Med. Imag."}$/;"	s
IEEE_J_MI	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_MI         = "{IEEE} Transactions on Medical Imaging"}$/;"	s
IEEE_J_MIL	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_MIL        = "{IEEE} Trans. Mil. Electron."}$/;"	s
IEEE_J_MIL	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_MIL        = "{IEEE} Transactions on Military Electronics"}$/;"	s
IEEE_J_MM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_MM         = "{IEEE} Trans. Multimedia"}$/;"	s
IEEE_J_MM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_MM         = "{IEEE} Transactions on Multimedia"}$/;"	s
IEEE_J_MMS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_MMS        = "{IEEE} Trans. Man-Mach. Syst."}$/;"	s
IEEE_J_MMS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_MMS        = "{IEEE} Transactions on Man-Machine Systems"}$/;"	s
IEEE_J_MTT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_MTT        = "{IEEE} Trans. Microw. Theory Tech."}$/;"	s
IEEE_J_MTT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_MTT        = "{IEEE} Transactions on Microwave Theory and Techniques"}$/;"	s
IEEE_J_MWCL	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_MWCL       = "{IEEE} Microw. Wireless Compon. Lett."}$/;"	s
IEEE_J_MWCL	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_MWCL       = "{IEEE} Microwave and Wireless Components Letters"}$/;"	s
IEEE_J_NANO	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_NANO       = "{IEEE} Trans. Nanotechnol."}$/;"	s
IEEE_J_NANO	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_NANO       = "{IEEE} Transactions on Nanotechnology"}$/;"	s
IEEE_J_NB	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_NB         = "{IEEE} Trans. Nanobiosci."}$/;"	s
IEEE_J_NB	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_NB         = "{IEEE} Transactions on NanoBioscience"}$/;"	s
IEEE_J_NET	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_NET        = "{IEEE\/ACM} Trans. Netw."}$/;"	s
IEEE_J_NET	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_NET        = "{IEEE\/ACM} Transactions on Networking"}$/;"	s
IEEE_J_NN	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_NN         = "{IEEE} Trans. Neural Netw."}$/;"	s
IEEE_J_NN	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_NN         = "{IEEE} Transactions on Neural Networks"}$/;"	s
IEEE_J_NS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_NS         = "{IEEE} Trans. Nucl. Sci."}$/;"	s
IEEE_J_NS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_NS         = "{IEEE} Transactions on Nuclear Science"}$/;"	s
IEEE_J_NSRE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_NSRE       = "{IEEE} Trans. Neural Syst. Rehabil. Eng."}$/;"	s
IEEE_J_NSRE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_NSRE       = "{IEEE} Transactions on Neural Systems and Rehabilitation Engineerin/;"	s
IEEE_J_OE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_OE         = "{IEEE} J. Ocean. Eng."}$/;"	s
IEEE_J_OE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_OE         = "{IEEE} Journal of Oceanic Engineering"}$/;"	s
IEEE_J_PAMI	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PAMI       = "{IEEE} Trans. Pattern Anal. Mach. Intell."}$/;"	s
IEEE_J_PAMI	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PAMI       = "{IEEE} Transactions on Pattern Analysis and Machine Intelligence"}$/;"	s
IEEE_J_PC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PC         = "{IEEE} Trans. Prof. Commun."}$/;"	s
IEEE_J_PC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PC         = "{IEEE} Transactions on Professional Communication"}$/;"	s
IEEE_J_PDS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PDS        = "{IEEE} Trans. Parallel Distrib. Syst."}$/;"	s
IEEE_J_PDS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PDS        = "{IEEE} Transactions on Parallel and Distributed Systems"}$/;"	s
IEEE_J_PEL	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PEL        = "{IEEE} Power Electron. Lett."}$/;"	s
IEEE_J_PEL	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PEL        = "{IEEE} Power Electronics Letters"}$/;"	s
IEEE_J_PHP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PHP        = "{IEEE} Trans. Parts, Hybrids, Packag."}$/;"	s
IEEE_J_PHP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PHP        = "{IEEE} Transactions on Parts, Hybrids and Packaging"}$/;"	s
IEEE_J_PMP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PMP        = "{IEEE} Trans. Parts, Mater., Packag."}$/;"	s
IEEE_J_PMP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PMP        = "{IEEE} Transactions on Parts, Materials and Packaging"}$/;"	s
IEEE_J_PROC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PROC       = "Proc. {IEEE}"}$/;"	s
IEEE_J_PROC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PROC       = "Proceedings of the {IEEE}"}$/;"	s
IEEE_J_PS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PS         = "{IEEE} Trans. Plasma Sci."}$/;"	s
IEEE_J_PS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PS         = "{IEEE} Transactions on Plasma Science"}$/;"	s
IEEE_J_PSE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PSE        = "{IEEE} J. Product Safety Eng."}$/;"	s
IEEE_J_PSE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PSE        = "{IEEE} Journal of Product Safety Engineering"}$/;"	s
IEEE_J_PTL	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PTL        = "{IEEE} Photon. Technol. Lett."}$/;"	s
IEEE_J_PTL	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PTL        = "{IEEE} Photonics Technology Letters"}$/;"	s
IEEE_J_PWRAS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PWRAS      = "{IEEE} Trans. Power App. Syst."}$/;"	s
IEEE_J_PWRAS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PWRAS      = "{IEEE} Transactions on Power Apparatus and Systems"}$/;"	s
IEEE_J_PWRD	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PWRD       = "{IEEE} Trans. Power Del."}$/;"	s
IEEE_J_PWRD	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PWRD       = "{IEEE} Transactions on Power Delivery"}$/;"	s
IEEE_J_PWRE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PWRE       = "{IEEE} Trans. Power Electron."}$/;"	s
IEEE_J_PWRE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PWRE       = "{IEEE} Transactions on Power Electronics"}$/;"	s
IEEE_J_PWRS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_PWRS       = "{IEEE} Trans. Power Syst."}$/;"	s
IEEE_J_PWRS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_PWRS       = "{IEEE} Transactions on Power Systems"}$/;"	s
IEEE_J_R	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_R          = "{IEEE} Trans. Rel."}$/;"	s
IEEE_J_R	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_R          = "{IEEE} Transactions on Reliability"}$/;"	s
IEEE_J_RA	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_RA         = "{IEEE} Trans. Robot. Autom."}$/;"	s
IEEE_J_RA	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_RA         = "{IEEE} Transactions on Robotics and Automation"}$/;"	s
IEEE_J_RE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_RE         = "{IEEE} Trans. Rehabil. Eng."}$/;"	s
IEEE_J_RE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_RE         = "{IEEE} Transactions on Rehabilitation Engineering"}$/;"	s
IEEE_J_RFI	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_RFI        = "{IEEE} Trans. Radio Freq. Interference"}$/;"	s
IEEE_J_RFI	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_RFI        = "{IEEE} Transactions on Radio Frequency Interference"}$/;"	s
IEEE_J_RO	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_RO         = "{IEEE} Trans. Robot."}$/;"	s
IEEE_J_RO	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_RO         = "{IEEE} Transactions on Robotics"}$/;"	s
IEEE_J_SAP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_SAP        = "{IEEE} Trans. Speech Audio Process."}$/;"	s
IEEE_J_SAP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_SAP        = "{IEEE} Transactions on Speech and Audio Processing"}$/;"	s
IEEE_J_SE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_SE         = "{IEEE} Trans. Softw. Eng."}$/;"	s
IEEE_J_SE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_SE         = "{IEEE} Transactions on Software Engineering"}$/;"	s
IEEE_J_SENSOR	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_SENSOR     = "{IEEE} Sensors J."}$/;"	s
IEEE_J_SENSOR	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_SENSOR     = "{IEEE} Sensors Journal"}$/;"	s
IEEE_J_SM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_SM         = "{IEEE} Trans. Semicond. Manuf."}$/;"	s
IEEE_J_SM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_SM         = "{IEEE} Transactions on Semiconductor Manufacturing"}$/;"	s
IEEE_J_SMC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_SMC        = "{IEEE} Trans. Syst., Man, Cybern."}$/;"	s
IEEE_J_SMC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_SMC        = "{IEEE} Transactions on Systems, Man, and Cybernetics"}$/;"	s
IEEE_J_SMCA	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_SMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}$/;"	s
IEEE_J_SMCA	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_SMCA       = "{IEEE} Transactions on Systems, Man, and Cybernetics---Part {A}: Sy/;"	s
IEEE_J_SMCB	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_SMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}$/;"	s
IEEE_J_SMCB	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_SMCB       = "{IEEE} Transactions on Systems, Man, and Cybernetics---Part {B}: Cy/;"	s
IEEE_J_SMCC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_SMCC       = "{IEEE} Trans. Syst., Man, Cybern. {C}"}$/;"	s
IEEE_J_SMCC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_SMCC       = "{IEEE} Transactions on Systems, Man, and Cybernetics---Part {C}: Ap/;"	s
IEEE_J_SP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_SP         = "{IEEE} Trans. Signal Process."}$/;"	s
IEEE_J_SP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_SP         = "{IEEE} Transactions on Signal Processing"}$/;"	s
IEEE_J_SPL	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_SPL        = "{IEEE} Signal Process. Lett."}$/;"	s
IEEE_J_SPL	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_SPL        = "{IEEE} Signal Processing Letters"}$/;"	s
IEEE_J_SSC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_SSC        = "{IEEE} Trans. Syst. Sci. Cybern."}$/;"	s
IEEE_J_SSC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_SSC        = "{IEEE} Transactions on Systems Science and Cybernetics"}$/;"	s
IEEE_J_SU	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_SU         = "{IEEE} Trans. Sonics Ultrason."}$/;"	s
IEEE_J_SU	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_SU         = "{IEEE} Transactions on Sonics and Ultrasonics"}$/;"	s
IEEE_J_TCAD	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_TCAD       = "{IEEE} J. Technol. Comput. Aided Design"}$/;"	s
IEEE_J_TCAD	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_TCAD       = "{IEEE} Journal on Technology in Computer Aided Design"}$/;"	s
IEEE_J_TJMJ	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_TJMJ       = "{IEEE} Transl. J. Magn. Jpn."}$/;"	s
IEEE_J_TJMJ	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_TJMJ       = "{IEEE} Translation Journal on Magnetics in Japan"}$/;"	s
IEEE_J_UE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_UE         = "{IEEE} Trans. Ultrason. Eng."}$/;"	s
IEEE_J_UE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_UE         = "{IEEE} Transactions on Ultrasonics Engineering"}$/;"	s
IEEE_J_UFFC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_UFFC       = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}$/;"	s
IEEE_J_UFFC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_UFFC       = "{IEEE} Transactions on Ultrasonics, Ferroelectrics, and Frequency C/;"	s
IEEE_J_VC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_VC         = "{IEEE} Trans. Veh. Commun."}$/;"	s
IEEE_J_VC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_VC         = "{IEEE} Transactions on Vehicular Communications"}$/;"	s
IEEE_J_VCG	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_VCG        = "{IEEE} Trans. Vis. Comput. Graphics"}$/;"	s
IEEE_J_VCG	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_VCG        = "{IEEE} Transactions on Visualization and Computer Graphics"}$/;"	s
IEEE_J_VLSI	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_VLSI       = "{IEEE} Trans. {VLSI} Syst."}$/;"	s
IEEE_J_VLSI	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_VLSI       = "{IEEE} Transactions on Very Large Scale Integration ({VLSI}) System/;"	s
IEEE_J_VT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_VT         = "{IEEE} Trans. Veh. Technol."}$/;"	s
IEEE_J_VT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_VT         = "{IEEE} Transactions on Vehicular Technology"}$/;"	s
IEEE_J_WCOM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_J_WCOM       = "{IEEE} Trans. Wireless Commun."}$/;"	s
IEEE_J_WCOM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_J_WCOM       = "{IEEE} Transactions on Wireless Communications"}$/;"	s
IEEE_M_AES	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_AES        = "{IEEE} Aerosp. Electron. Syst. Mag."}$/;"	s
IEEE_M_AES	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_AES        = "{IEEE} Aerospace and Electronics Systems Magazine"}$/;"	s
IEEE_M_AP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_AP         = "{IEEE} Antennas Propag. Mag."}$/;"	s
IEEE_M_AP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_AP         = "{IEEE} Antennas and Propagation Magazine"}$/;"	s
IEEE_M_ASSP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Mag."}$/;"	s
IEEE_M_ASSP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Magazine"}$/;"	s
IEEE_M_C	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_C          = "{IEEE} Computer"}$/;"	s
IEEE_M_C	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_C          = "{IEEE} Computer"}$/;"	s
IEEE_M_CAP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_CAP        = "{IEEE} Comput. Appl. Power"}$/;"	s
IEEE_M_CAP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_CAP        = "{IEEE} Computer Applications in Power"}$/;"	s
IEEE_M_CAS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_CAS        = "{IEEE} Circuits Syst. Mag."}$/;"	s
IEEE_M_CAS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_CAS        = "{IEEE} Circuits and Systems Magazine"}$/;"	s
IEEE_M_CD	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_CD         = "{IEEE} Circuits Devices Mag."}$/;"	s
IEEE_M_CD	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_CD         = "{IEEE} Circuits and Devices Magazine"}$/;"	s
IEEE_M_CGA	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_CGA        = "{IEEE} Comput. Graph. Appl."}$/;"	s
IEEE_M_CGA	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_CGA        = "{IEEE} Computer Graphics and Applications"}$/;"	s
IEEE_M_CIM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_CIM        = "{IEEE} Comput. Intell. Mag."}$/;"	s
IEEE_M_CIM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_CIM        = "{IEEE} Computational Intelligence Magazine"}$/;"	s
IEEE_M_COM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_COM        = "{IEEE} Commun. Mag."}$/;"	s
IEEE_M_COM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_COM        = "{IEEE} Communications Magazine"}$/;"	s
IEEE_M_COMSOC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_COMSOC     = "{IEEE} Commun. Soc. Mag."}$/;"	s
IEEE_M_COMSOC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_COMSOC     = "{IEEE} Communications Society Magazine"}$/;"	s
IEEE_M_CONC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}$/;"	s
IEEE_M_CONC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}$/;"	s
IEEE_M_CS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_CS         = "{IEEE} Control Syst. Mag."}$/;"	s
IEEE_M_CS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_CS         = "{IEEE} Control Systems Magazine"}$/;"	s
IEEE_M_CSE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_CSE        = "{IEEE} Comput. Sci. Eng."}$/;"	s
IEEE_M_CSE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_CSE        = "{IEEE} Computing in Science and Engineering"}$/;"	s
IEEE_M_CSEM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_CSEM       = "{IEEE} Comput. Sci. Eng. Mag."}$/;"	s
IEEE_M_CSEM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_CSEM       = "{IEEE} Computational Science and Engineering Magazine"}$/;"	s
IEEE_M_DTC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_DTC        = "{IEEE} Des. Test. Comput."}$/;"	s
IEEE_M_DTC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_DTC        = "{IEEE} Design and Test of Computers"}$/;"	s
IEEE_M_EI	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_EI         = "{IEEE} Electr. Insul. Mag."}$/;"	s
IEEE_M_EI	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_EI         = "{IEEE} Electrical Insulation Magazine"}$/;"	s
IEEE_M_EMB	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_EMB        = "{IEEE} Eng. Med. Biol. Mag."}$/;"	s
IEEE_M_EMB	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_EMB        = "{IEEE} Engineering in Medicine and Biology Magazine"}$/;"	s
IEEE_M_EMR	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_EMR        = "{IEEE} Eng. Manag. Rev."}$/;"	s
IEEE_M_EMR	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_EMR        = "{IEEE} Engineering Management Review"}$/;"	s
IEEE_M_ETR	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_ETR        = "{IEEE} ElectroTechnol. Rev."}$/;"	s
IEEE_M_ETR	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_ETR        = "{IEEE} ElectroTechnology Review"}$/;"	s
IEEE_M_EXP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_EXP        = "{IEEE} Expert"}$/;"	s
IEEE_M_EXP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_EXP        = "{IEEE} Expert"}$/;"	s
IEEE_M_HIST	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_HIST       = "{IEEE} Ann. Hist. Comput."}$/;"	s
IEEE_M_HIST	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_HIST       = "{IEEE} Annals of the History of Computing"}$/;"	s
IEEE_M_IA	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_IA         = "{IEEE} Ind. Appl. Mag."}$/;"	s
IEEE_M_IA	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_IA         = "{IEEE} Industry Applications Magazine"}$/;"	s
IEEE_M_IC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_IC         = "{IEEE} Internet Comput."}$/;"	s
IEEE_M_IC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_IC         = "{IEEE} Internet Computing"}$/;"	s
IEEE_M_IM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_IM         = "{IEEE} Instrum. Meas. Mag."}$/;"	s
IEEE_M_IM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_IM         = "{IEEE} Instrumentation and Measurement Magazine"}$/;"	s
IEEE_M_IS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_IS         = "{IEEE} Intell. Syst."}$/;"	s
IEEE_M_IS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_IS         = "{IEEE} Intelligent Systems"}$/;"	s
IEEE_M_ITP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_ITP        = "{IEEE} {IT} Prof."}$/;"	s
IEEE_M_ITP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_ITP        = "{IEEE} {IT} Professional"}$/;"	s
IEEE_M_MICRO	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_MICRO      = "{IEEE} Micro"}$/;"	s
IEEE_M_MICRO	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_MICRO      = "{IEEE} Micro"}$/;"	s
IEEE_M_MM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_MM         = "{IEEE} Multimedia"}$/;"	s
IEEE_M_MM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_MM         = "{IEEE} Multimedia"}$/;"	s
IEEE_M_MW	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_MW         = "{IEEE} Microw. Mag."}$/;"	s
IEEE_M_MW	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_MW         = "{IEEE} Microwave Magazine"}$/;"	s
IEEE_M_NET	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_NET        = "{IEEE} Netw."}$/;"	s
IEEE_M_NET	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_NET        = "{IEEE} Network"}$/;"	s
IEEE_M_PCOM	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_PCOM       = "{IEEE} Personal Commun. Mag."}$/;"	s
IEEE_M_PCOM	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_PCOM       = "{IEEE} Personal Communications Magazine"}$/;"	s
IEEE_M_PE	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_PE         = "{IEEE} Power Energy Mag."}$/;"	s
IEEE_M_PE	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_PE         = "{IEEE} Power and Energy Magazine"}$/;"	s
IEEE_M_PER	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_PER        = "{IEEE} Power Eng. Rev."}$/;"	s
IEEE_M_PER	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_PER        = "{IEEE} Power Engineering Review"}$/;"	s
IEEE_M_POT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_POT        = "{IEEE} Potentials"}$/;"	s
IEEE_M_POT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_POT        = "{IEEE} Potentials"}$/;"	s
IEEE_M_PVC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_PVC        = "{IEEE} Pervasive Comput."}$/;"	s
IEEE_M_PVC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_PVC        = "{IEEE} Pervasive Computing"}$/;"	s
IEEE_M_RA	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_RA         = "{IEEE} Robot. Autom. Mag."}$/;"	s
IEEE_M_RA	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_RA         = "{IEEE} Robotics and Automation Magazine"}$/;"	s
IEEE_M_S	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_S          = "{IEEE} Softw."}$/;"	s
IEEE_M_S	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_S          = "{IEEE} Software"}$/;"	s
IEEE_M_SAP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_SAP        = "{IEEE} Security Privacy"}$/;"	s
IEEE_M_SAP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_SAP        = "{IEEE} Security and Privacy"}$/;"	s
IEEE_M_SP	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_SP         = "{IEEE} Signal Process. Mag."}$/;"	s
IEEE_M_SP	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_SP         = "{IEEE} Signal Processing Magazine"}$/;"	s
IEEE_M_SPECT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_SPECT      = "{IEEE} Spectr."}$/;"	s
IEEE_M_SPECT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_SPECT      = "{IEEE} Spectrum"}$/;"	s
IEEE_M_TODAY	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_TODAY      = "Today's Engineer"}$/;"	s
IEEE_M_TODAY	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_TODAY      = "Today's Engineer"}$/;"	s
IEEE_M_TS	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_TS         = "{IEEE} Technol. Soc. Mag."}$/;"	s
IEEE_M_TS	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_TS         = "{IEEE} Technology and Society Magazine"}$/;"	s
IEEE_M_VT	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_VT         = "{IEEE} Veh. Technol. Mag."}$/;"	s
IEEE_M_VT	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_VT         = "{IEEE} Vehicular Technology Magazine"}$/;"	s
IEEE_M_WC	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_M_WC         = "{IEEE} Wireless Commun. Mag."}$/;"	s
IEEE_M_WC	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_M_WC         = "{IEEE} Wireless Communications Magazine"}$/;"	s
IEEE_O_CSTO	IEEEtranBST2/IEEEabrv.bib	/^@STRING{IEEE_O_CSTO        = "{IEEE} Commun. Surveys Tuts."}$/;"	s
IEEE_O_CSTO	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_O_CSTO        = "{IEEE} Communications Surveys and Tutorials"}$/;"	s
IEEE_O_DSO	IEEEtranBST2/IEEEfull.bib	/^@STRING{IEEE_O_DSO         = "{IEEE} Distributed Systems Online"}$/;"	s
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@article{IEEEexample:TBParticle,$/;"	a
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@article{IEEEexample:article_typical,$/;"	a
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@article{IEEEexample:articledualmonths,$/;"	a
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@article{IEEEexample:articleetal,$/;"	a
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@article{IEEEexample:articlelargepages,$/;"	a
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@article{IEEEexample:bluebookarticle,$/;"	a
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@book{IEEEexample:bluebookbook,$/;"	b
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@book{IEEEexample:book,$/;"	b
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@book{IEEEexample:book_typical,$/;"	b
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@book{IEEEexample:bookwitheditor,$/;"	b
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@book{IEEEexample:bookwithseriesvolume,$/;"	b
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@inbook{IEEEexample:inbook,$/;"	i
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@inbook{IEEEexample:inbookpagesnote,$/;"	i
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@incollection{IEEEexample:incollection,$/;"	I
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@incollection{IEEEexample:incollection_chpp,$/;"	I
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@incollection{IEEEexample:incollectionmanyauthors,$/;"	I
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@incollection{IEEEexample:incollectionwithseries,$/;"	I
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@inproceedings{IEEEexample:conf_typical,$/;"	j
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@inproceedings{IEEEexample:confwithadddays,$/;"	j
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@inproceedings{IEEEexample:confwithpaper,$/;"	j
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@inproceedings{IEEEexample:confwithpapertype,$/;"	j
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@inproceedings{IEEEexample:confwithvolume,$/;"	j
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@inproceedings{IEEEexample:presentedatconf,$/;"	j
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@manual{IEEEexample:bluebookmanual,$/;"	m
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@manual{IEEEexample:motmanual,$/;"	m
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@manual{IEEEexample:motmanualhowpub,$/;"	m
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@manual{IEEEexample:softmanual,$/;"	m
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@mastersthesis{IEEEexample:masters,$/;"	M
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@mastersthesis{IEEEexample:masterstype,$/;"	M
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@misc{IEEEexample:TBPmisc,$/;"	n
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@misc{IEEEexample:datasheet,$/;"	n
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@misc{IEEEexample:draftasmisc,$/;"	n
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@misc{IEEEexample:miscforum,$/;"	n
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@misc{IEEEexample:miscgermanreg,$/;"	n
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@misc{IEEEexample:miscrfc,$/;"	n
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@misc{IEEEexample:private,$/;"	n
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@misc{IEEEexample:whitepaper,$/;"	n
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@phdthesis{IEEEexample:phdurl,$/;"	p
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@techreport{IEEEexample:techrep,$/;"	t
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@techreport{IEEEexample:techreptype,$/;"	t
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@techreport{IEEEexample:techreptypeii,$/;"	t
IEEEexample	IEEEtranBST2/IEEEexample.bib	/^@unpublished{IEEEexample:unpublished,$/;"	u
Introduction	main.tex	/^\\section{Introduction}$/;"	s
test	bibliography.bib	/^@article{test,$/;"	a

